Multidimensional Interleavings and Applications to Topological Inference

This work concerns the theoretical foundations of persistence-based topological data analysis. We develop theory of topological inference in the multidimensional persistence setting, and directly at the (topological) level of filtrations rather than only at the (algebraic) level of persistent homology modules. Our main mathematical objects of study are interleavings. These are tools for quantifying the similarity between two multidimensional filtrations or persistence modules. They were introduced for 1-D filtrations and persistence modules by Chazal, Cohen-Steiner, Glisse, Guibas, and Oudot. We introduce generalizations of the definitions of interleavings given by Chazal et al. and use these to define pseudometrics, called interleaving distances, on multidimensional filtrations and multidimensional persistence modules. We present an in-depth study of interleavings and interleaving distances. We then use them to formulate and prove several multidimensional analogues of a topological inference theorem of Chazal, Guibas, Oudot, and Skraba. These results hold directly at the level of filtrations; they yield as corollaries corresponding results at the module level.

==> Part_I/T_Paper_Discussion.tex <==
\section{Discussion of Future Work}\label{DiscussionSection}

We believe that Theorem~\ref{InterleavingEqualsBottleneck}, Corollary~\ref{MetricCorollary}, and Corollary~\ref{CorOptimality} establish the credentials of the interleaving distance as a natural generalization of the bottleneck distance to the setting of multidimensional persistence.

Insofar as the interleaving distance is in fact a good choice of distance on multidimensional persistence modules, the question of how to compute it is interesting and important from the standpoint of applications.  One obvious potential application of interleaving distance computations is to shape matching.  Other potential applications of a more statistical nature are discussed in Section~\ref{}.   

The results of Section~\ref{ComputationSection} suggest a path towards the development of a theory of computation of the interleaving distance.  We plan to pursue this path further in subsequent work.  As noted in Section~\ref{ComputationSection}, to exploit the connection with multivariate quadratics in the development of such a theory in practice, one needs in particular a way of computing minimal presentations of simplicial homology modules of simplicial $n$-filtrations.  We will address this problem in a companion paper. %\cite{ComputingMinimalPresentations}.  

As mentioned in the introduction, our view is that the existence of a good choice of pseudometric on multidimensional persistence modules promises to facilitate the adaptation to the multidimensional setting of theoretical results and applications of ordinary persistence which depend on the bottleneck distance.  We believe that there is plenty of interesting and potentially useful work to be done in carrying out this adaptation.

Corollary~\ref{CorOptimality} demonstrates that the interleaving distance is optimal in the sense of Example~\ref{AllDimsSublevelsetEx} when $k=\Q$ or $\Z/p\Z$.  However, our discussion of optimality of pseudometrics in Section~\ref{OptimalityGeneralities} raises many more questions than it answers.  Some of the more interesting questions are:

\begin{enumerate*}
\item Can we extend the result of Theorem~\ref{MainOptimality} to arbitrary ground fields?  %It seems this would involve invoking an analogue of the universal coefficient theorem for persistence.
\item Can we extend the result of Theorem~\ref{MainOptimality} to the case $i=0$?  
\item Can we prove that the interleaving distance is ${\mathcal R}$-optimal for ${\mathcal R}$ any of the relative structures on $\obj^*(B_n$-mod$)$ defined in Examples~\ref{SublevelsetOffsetOptimality}-\ref{VariantExample}?  The case of Example~\ref{SublevelsetRipsOptimality} is of particular interest to us.  We have observed in Section~\ref{InducedSemiPseudometrics} that in this case an ${\mathcal R}$-optimal pseudometric does exist.    
\item\label{Generalizations} Can we obtain analogous results about the optimality of pseudometrics on more general types of persistent homology modules?  For instance, can we prove a result analogous to Theorem~\ref{MainOptimality} for levelset zigzag persistence \cite{carlsson2009zigzag}?
\end{enumerate*}

An interesting question related to question~\ref{Generalizations} above is whether there is a way of algebraically reformulating the bottleneck distance for zigzag persistence modules as an analogue of the interleaving distance in such way that the definition generalizes to a larger classes of quiver representations \cite{derksen2005quiver}.

%Our optimality result singles out the interleaving distance as the best pseudometric on multidimensional persistence modules, in a certain sense.  However, it is also interesting to ask whether the interleaving metric is completely characterized (up to multiplication by a scalar) by its stability and the property that it restricts to a metric on finitely presented $B_n$-modules.  

Finally, we mention again that it would be nice to have an extension of Theorem~\ref{WellBehavedStructureThm} to a structure theorem for arbitrary tame $B_1$-persistence modules, and an extension of Corollary~\ref{MetricCorollary} to well behaved tame $B_n$-persistence modules. %though it's not clear that such results would be particularly important from the standpoint of applications.  
